Distributionally Robust Counterfactual Risk Minimization

This manuscript introduces the idea of using Distributionally Robust Optimization (DRO) for the Counterfactual Risk Minimization (CRM) problem. Tapping into a rich existing literature, we show that DRO is a principled tool for counterfactual decision making. We also show that well-established solutions to the CRM problem like sample variance penalization schemes are special instances of a more general DRO problem. In this unifying framework, a variety of distributionally robust counterfactual risk estimators can be constructed using various probability distances and divergences as uncertainty measures. We propose the use of Kullback-Leibler divergence as an alternative way to model uncertainty in CRM and derive a new robust counterfactual objective. In our experiments, we show that this approach outperforms the state-of-the-art on four benchmark datasets, validating the relevance of using other uncertainty measures in practical applications.

==> blbf_aaai.tex <==
\section{Batch Learning from Logged Bandit Feedback}
\label{sec:blbf}

\subsection{Notation and terminology}
We denote $x\in\mX$ arbitrary \emph{contexts} drawn from an unknown distribution $\nu$ and presented to the decision maker. Such a quantity can describe covariate information about a patient for a clinical test, or a potential targeted user in a recommender system. The variable $y\in\mY$ denotes the \emph{actions} available to the decision maker - the potential medications to give to the patient, or possible advertisements targeting the user for instance. A \emph{policy} is a mapping $\pi:\mX\to\mP\left(\mY\right)$ from the space of contexts to probabilities in the action space. For a given (context, action) pair $(x,y)$, the quantity $\pi(y\vert x)$ denotes the probability of the policy $\pi$ to take the action $y$ when presented the context $x$. When picking the action $y$ for a given context $x$, the decision maker receives a \emph{reward} $\delta(x,y)$, drawn from an unknown distribution. In our examples, this reward could indicate a patient's remission, or the fact that the targeted user clicked on the displayed ad. This reward $\delta(x,y)$ can also be assumed to be deterministic - as in \cite{swaminathan2015batch,swaminathan2015self}. We make this assumption in the rest of this manuscript. Finally, for a given context $x \in \mathcal{X}$ and an action $y \in \mathcal{Y}$, we define the cost function $c(x,y) \triangleq - \delta(x,y)$.

In this paper, we try to find policies producing low expected costs. To make this search tractable, it is usual to restrict the search to a family of \emph{parametric} policies, henceforth tying policies $\pi_\theta$ to a vector $\theta\in\Theta$. The $\emph{risk}$:
\begin{align}
    R(\theta) \triangleq \bE_{x\sim \nu, y\sim \pi_\theta(\cdot\vert x)}\left[ c(x,y) \right] 
\end{align} corresponds to the expected cost obtained by the policy $\pi_\theta$ through the different actions $y$ taken, a quantity the decision maker will try to minimize.

\subsection{Counterfactual Risk Minimization}
\label{subsec:crm}
%\paragraph{Batch Learning from Bandit Feedback}
In practical applications, it is common that one has only access to the \emph{interaction logs} of a previous version of the decision making system, also called a \emph{logging policy} (denoted $\pi_0$). More formally, we are interested in the case where the only available data is a collection of quadruplets $\mH\triangleq \left(x_i ,y_i, p_i, c_i\right)_{1\leq i \leq n}$, where the costs $c_i \triangleq c(x_i, y_i)$ were obtained after taking an action $y_i$ with probability $p_i\triangleq \pi_0(y_i\vert x_i)$ when presented with a context $x_i \sim \nu$.

%\paragraph{Counterfactual estimators}
In order to search for policies $\pi_\theta$ with smaller risk than $\pi_0$, one needs to build counterfactual estimators for $R(\theta)$ from the historic $\mH$. One way to do so is to use \emph{inverse propensity scores} \cite{rosenblum1983central}:
\begin{equation}
    \begin{aligned}
    R(\theta) &= \bE_{x\sim \nu, y\sim \pi_\theta(x)}\left[ c(x,y) \right]\\
                    &=  \bE_{x \sim \nu, y \sim \pi_0(x)}\left[ c(x,y) \frac{\pi_\theta(y\vert x)}{\pi_0(y\vert x)} \right]
\label{eq:ips_risk} 
\end{aligned}
\end{equation}
for any $\pi_\theta$ absolutely continuous w.r.t $\pi_0$.
Henceforth, $R(\theta)$ can be approximated with samples $(x_i, y_i, p_i,c_i)$ from the interaction logs $\mH$ via the sample average approximation:
\begin{align}
    R(\theta) \simeq \frac{1}{n}\sum_{i=1}^n c_i\frac{\pi_\theta(y_i\vert x_i)}{p_i}
    \label{eq:ips_empirical_risk}
\end{align}

Bluntly minimizing the objective provided by the counterfactual risk estimator \eqref{eq:ips_empirical_risk} is known to be sub-optimal, as it can have \emph{unbounded} variance \cite{ionides2008truncated}. It is therefore a classical technique \cite{bottou2013counterfactual,cortes2010learning,strehl2010learning,swaminathan2015batch} to \emph{clip} the propensity weights . This leads to the Clipped Inverse Propensity Scores (CIPS) estimator:
\begin{align}
    \hat{R}_n(\theta) \triangleq \frac{1}{n}\sum_{i=1}^n c_i \min\left(M, \frac{\pi_\theta(y_i\vert x_i)}{p_i}\right).
    \label{eq:empirical_clipped}
\end{align}
The variable $M$ is an hyper-parameter, balancing the variance reduction brought by weight clipping and the bias introduced in the empirical estimation of $R(\theta)$. The search for a minimal $\theta$ with respect to the estimator $\hat{R}_n(\theta)$ is often referred to as \emph{Counterfactual Risk Minimization} (CRM). 

\paragraph{Remark 1} Other techniques have been proposed in the literature to reduce the variance of the risk estimators. For instance, the doubly robust risk \cite{dudik2011doubly} takes advantage of both counterfactual estimators and supervised learning methods, while the self-normalized risk \cite{swaminathan2015self} was designed to counter the effect of a phenomenon known as propensity overfitting. We do not explicitly cover them in our analysis, but the results we derive hereinafter also hold for such estimators.


% We discuss in this paper the design of robustified counterfactual estimator for the clipped propensity risk \eqref{eq:ips_empirical_risk}, as in \cite{bottou2013counterfactual, swaminathan2015batch, swaminathan2015batch} and showed its link with sample variance penalized objective. Other risk estimators have been proposed, namely by the authors of \cite{swaminathan2015self} who introduce the \emph{self-normalized} counterfactual risk to counter a phenomenon called \emph{propensity overfitting}. 
%\paragraph{Additional notations} To ease notations, we introduce the variable $z^\pi(x,y) \triangleq c(x,y) \min\left\{M, \frac{\pi(y\vert x)}{\pi_0(y\vert x)}\right\}$. We therefore have by definition the following relationships:
%\begin{subequations}
%    \begin{align}
%        R^M(\pi) &= \bE_{x \sim \nu, y \sim \pi_0(x) }\left[z^\pi(x,y)\right]\\
%        \hat{R}^M_n(\pi) &=\frac{1}{n}\sum_{i=1}^n z^\pi(x_i,y_i)
%    \end{align}
%\end{subequations}

\subsection{Sample-Variance Penalization}

The main drawback of the CIPS estimator is that two different policies can have risk estimates of highly different variance - something the sample average approximation cannot capture. The authors of \cite{swaminathan2015batch} developed a variance-sensitive action selection process where one penalizes policies with high-variance risk estimates. Their approach is based on a sample-variance penalized version of the CIPS estimator:
\begin{align}
    \hat{R}_n^{\lambda} (\theta) \triangleq \hat{R}_n(\theta) + \lambda \sqrt{V_n(\theta)/n},
    \label{eq:poem_obj}
\end{align}
where $\lambda$ is an hyper-parameter set by the practitioner, and $V_n(\theta)$ denotes the empirical variance of the quantities $c_i \min\left(M, \frac{\pi_\theta(y_i \vert x_i)}{p_i}\right)$. The main motivation behind this approach is based on confidence bounds derived in \cite{maurer09}, upper-bounding with high-probability the true risk $R(\theta)$ by the empirical risk $\hat{R}_n(\theta)$ augmented with an  additive empirical variance term. In a few words, this allows to build and optimize a pessimistic envelope for the true risk and penalize policies with high variance risk estimates. The authors of \cite{swaminathan2015batch} proposed the Policy Optimization for Exponential Models (POEM) algorithm and showed state-of-the-art results on a collection of counterfactual tasks when applying this method to exponentially parametrized policies:
\begin{eqnarray}
    \pi_\theta(y\vert x) \propto \exp\left( \theta^T \phi(x, y)\right),
    \label{eq:exponential_model}
\end{eqnarray}
with $\phi(x, y)$ being a $d$-dimensional joint feature map.

==> related.tex <==
\section{Related Work}\label{sec:related}

We discuss in this paper the design of robustified counterfactual estimator for the clipped propensity risk \eqref{eq:ips_empirical_risk}, as in \cite{bottou2013counterfactual, swaminathan2015batch, swaminathan2015batch} and showed its link with sample variance penalized objective. Other risk estimators have been proposed, namely by the authors of \cite{swaminathan2015self} who introduce the \emph{self-normalized} counterfactual risk to counter a phenomenon called \emph{propensity overfitting}. 
%Other solutions have been proposed building feedback oracles for unseen pairs of users and actions, moving the problem back to standard supervised learning \cite{beygelzimer2009offset, zadrozny2003cost}. 
